TEMPO: Temporally-grounded Multi-task Post-training for Large Audio-Language Models

Large audio-language models (LALMs) describe audio at the clip level but cannot assign timestamps to the events, speakers, or sounds they identify. Despite being essential for downstream tasks like speech recognition and dense audio captioning, timestamping remains a key limitation of most LALMs. We present TEMPO (Temporally-grounded Multi-task Post-training), the first unified model to handle audio, speech, and music timestamping tasks. Our core contribution is a supervised fine-tuning (SFT) stage built on three innovations: atomic timestamp tokens, a time-aware projector that injects sinusoidal wall-clock encodings into audio frame embeddings, and a distance-aware Gaussian loss. Our training is based on a synthetic-to-real curriculum. We further introduce, to our knowledge, the first application of reinforcement learning to unified audio timestamping, using GRPO with verifiable temporal rewards that directly optimize the evaluation objectives. Rather than serving as the primary source of performance gains, GRPO acts as a refinement stage on top of the SFT checkpoint, providing modest additional improvements. To support this work, we build a training dataset containing 119K samples and an evaluation benchmark containing 10K samples, drawn from established corpora across five tasks. On this benchmark, TEMPO outperforms Audio Flamingo Next and Qwen3-Omni, two state-of-the-art LALMs explicitly trained on timestamped data. Experiments confirm that SFT delivers most of these gains, with GRPO providing consistent but moderate refinements.

==> sec/training.tex <==
\section{Training}

\subsection{Synthetic data}

\subsection{Rewards}

\subsection{Evaluation}
Each task is scored along both a \emph{temporal} and a \emph{content} axis, isolating \emph{when} errors from \emph{what} errors.
%
For \textbf{ASR}, we report segment-aligned Word Error Rate (WER), computed by first greedily matching predicted segments to reference segments by temporal IoU and then averaging per-pair WER; mean temporal Intersection-over-Union (mIoU) over reference events, where unmatched references contribute zero; and boundary Mean Absolute Error (MAE) of matched start/end times in seconds.
%
For \textbf{diarization}, we report Diarization Error Rate (DER) via \texttt{pyannote.metrics} with its standard decomposition into missed speech, false alarm, and speaker confusion; mIoU for pure temporal overlap; and speaker-labeled F1 at an IoU threshold of 0.5, which requires both temporal overlap and correct speaker identity, catching local label errors that DER's global optimal mapping can mask.
%
For \textbf{dense audio captioning}, we report segment-aligned METEOR, averaged over greedy IoU-matched prediction--reference pairs to isolate content quality given correct localization; mIoU for temporal localization; and event-level F1 at IoU${\geq}$0.5, which penalizes missed and spurious events.
% We additionally compute two complementary temporal metrics: Segment-based F1 (SegF1), which discretizes the timeline at 100\,ms resolution and micro-averages frame-level precision and recall across clips, and Event-based F1 (EvtF1) with a $\pm$1.0\,s onset collar, which performs greedy one-to-one onset matching to evaluate temporal localization independently of caption semantics.
%
For \textbf{audio grounding}, we report mIoU, detection F1 at IoU${\geq}$0.5, and boundary MAE; since this task has no textual payload, all three metrics are purely temporal.
%
For \textbf{music captioning}, we report chord mIoU (temporal overlap of chord segments), chord F1 at IoU${\geq}$0.5 (requiring both correct chord symbol and sufficient temporal overlap), and tempo accuracy within a 4\% tolerance.
%
Metrics where lower is better are WER, DER, and boundary MAE; all others are higher-is-better. Per-example scores are averaged across the evaluation set, with NaN values (e.g., boundary MAE when no segments are matched) excluded from aggregation.
